Spec2COBOLRot: An Agentic-AI Degradation Loop for Realistic COBOL Corpus Generation

COBOL remains widely deployed, yet representative corpora reflecting real production code are rarely available, limiting rigorous benchmarking of modernization approaches. We propose a systematic agentic AI pipeline for generating realistic COBOL programs, combining specification-driven generation with iterative degradation guided by patterns and complexity targets extracted from real production code. Here, realism is understood as structural fidelity to production code as captured by our metrics. We evaluate whether degradation reaches target complexity levels while preserving business behavior, and examine the limits of the approach, across three programs from distinct business domains. Results show the pipeline reliably produces syntactically valid programs and moves them toward realistic structural complexity. However, preserving business behavior is not always achieved by construction, and targeting structural metrics independently of business logic risks producing programs whose complexity does not reflect a plausible maintenance history. We discuss these limitations and outline a more realistic alternative as a direction for future work, generating legacy programs from scratch along a simulated development history.

==> old/asset-example.tex <==

\begin{figure}[t]
    \centering
    \begin{tcolorbox}
        [ colback=gray!5, colframe=gray!60, boxrule=0.4pt, arc=1pt, left=6pt, right=6pt,
        top=5pt, bottom=5pt, fontupper=\small ]

        \hspace{10pt}{\small\bfseries Explicit file-status checking}

        {\small\sffamily\bfseries\color{gray!70!black} (1) DESCRIPTION}
        \vspace{2pt}

        \hspace{10pt}
        \begin{minipage}{0.85\linewidth}
            \textit{``[\,\dots] check \texttt{FILE STATUS} after \texttt{OPEN},
            \texttt{READ}, \texttt{WRITE}, or \texttt{CLOSE} instead of assuming
            success. [\,\dots] common in programs that process several files or mix
            business validation with operational error handling.''}
        \end{minipage}

        \vspace{6pt}
        \hrule
        \vspace{6pt}

        {\small\sffamily\bfseries\color{gray!70!black} (2) CANONICAL FORM}
        \vspace{3pt}

        \hspace{10pt}
        \begin{minipage}{0.85\linewidth}
            \begin{verbatim}
    OPEN INPUT FCLIENT.
    IF FS-FCLIENT NOT = '00'
        MOVE 'ERR-OPEN-FCLIENT' TO WS-CODE-ERR
        PERFORM HANDLE-FATAL-FILE-ERROR
    END-IF.
\end{verbatim}
        \end{minipage}

        \vspace{6pt}
        \hrule
        \vspace{6pt}

        {\small\sffamily\bfseries\color{gray!70!black} (3) GENERATION GUIDANCE}
        \vspace{2pt}

        \hspace{10pt}
        \begin{minipage}{0.85\linewidth}
            \textit{``[\,\dots] injected when the program opens multiple files,
            performs critical writes, or must expose deterministic operator-visible
            failure paths. [\,\dots]''}
        \end{minipage}
    \end{tcolorbox}
    \caption{Excerpt of an asset from the idioms family: rationale, canonical
    code form, and generation guidance.} % used by the degradation agent.}
    \label{fig:asset-excerpt}
\end{figure}

==> old/spec-example.tex <==

\begin{figure}[t]
    \centering
    \begin{tcolorbox}
        [ colback=gray!5, colframe=gray!60, boxrule=0.4pt, arc=1pt, left=6pt, right=6pt,
        top=5pt, bottom=5pt, fontupper=\small ]

        {\small\sffamily\bfseries\color{gray!70!black} (1) FUNCTIONAL OBJECTIVE}
        \vspace{2pt}

        \textit{``[\,\dots] compute payroll for all employees active during the period,
        apply the employee and employer social contributions due, [\,\dots] and
        produce pay slips, the bank transfer file, and the statutory declaration.
        [\,\dots]''}

        \vspace{6pt}
        \hrule
        \vspace{6pt}

        {\small\sffamily\bfseries\color{gray!70!black} (2) INPUT DATA \hfill \footnotesize\normalfont\itshape\color{gray!50!black}}
        \vspace{4pt}

        \hspace{10pt}{\small\bfseries Employment contract} \hfill {\footnotesize\itshape\color{gray!50!black}}

        \vspace{3pt}
        \hspace{20pt}
        \begin{tabular}{@{}p{0.26\linewidth}p{0.58\linewidth}@{}}
            \textbf{Work-time ratio} & Proportion of full-time worked (\texttt{1.00} = full-time, e.g.\ \texttt{0.80} for 80\%). \\
        \end{tabular}

        \vspace{2pt}
        \hspace{20pt}{\footnotesize\itshape\color{gray!50!black}[\,\dots\ 8 more fields: base salary, seniority date, classification level, \dots]}

        \vspace{4pt}
        {\footnotesize\itshape\color{gray!50!black}[\,\dots\ 4 more data models: employee reference data, period movements, working calendar, employee tax profile]}

        \vspace{6pt}
        \hrule
        \vspace{6pt}

        {\small\sffamily\bfseries\color{gray!70!black} (3) OUTPUT DATA \hfill \footnotesize\normalfont\itshape\color{gray!50!black}}
        \vspace{4pt}

        \hspace{10pt}{\small\bfseries Pay slip} \hfill {\footnotesize\itshape\color{gray!50!black}}

        \vspace{3pt}
        \hspace{20pt}
        \begin{tabular}{@{}p{0.26\linewidth}p{0.58\linewidth}@{}}
            \textbf{Net pay} & Amount actually paid to the employee after all contributions and withholdings. Decimal amount. \\
        \end{tabular}

        \vspace{2pt}
        \hspace{20pt}{\footnotesize\itshape\color{gray!50!black}[\,\dots\ 9 more fields: gross pay, itemised contributions, taxable net, \dots]}

        \vspace{4pt}
        {\footnotesize\itshape\color{gray!50!black}[\,\dots\ 4 more data models: bank transfer file, statutory declaration, reject file, end-of-run report]}

        \vspace{6pt}
        \hrule
        \vspace{6pt}

        {\small\sffamily\bfseries\color{gray!70!black} (4) BUSINESS RULE \hfill \footnotesize\normalfont\itshape\color{gray!50!black}}
        \vspace{4pt}

        \hspace{10pt}{\small\bfseries Regular pay calculation}

        \vspace{3pt}
        \hspace{20pt}
        \begin{minipage}{0.85\linewidth}
            \begin{align*}
                \text{adjusted salary} & = \text{base salary}\times \textbf{\text{work-time ratio}} \\
                \text{regular pay}     & = \text{adjusted salary}- \text{absence deductions}
            \end{align*}

            \textit{Sick leave and unpaid leave are deducted at the daily rate; annual
            and statutory leave are paid, not deducted.}
        \end{minipage}

        \vspace{4pt}
        {\footnotesize\itshape\color{gray!50!black}[\,\dots\ 9 more rules: overtime tiers, contribution schedule, taxable net, \dots]}
    \end{tcolorbox}
    \caption{Excerpt from the PAYCOMBT specification (full Spec. defines
    5 inputs, 5 output, 10 business rules). The \textit{work-time
    ratio} field in (2) feeds directly into the calculation in (4).}
    \label{fig:spec-excerpt}
\end{figure}
